Jet energy calibration at the LHC

Jets are one of the most prominent physics signatures of high energy proton proton (p-p) collisions at the Large Hadron Collider (LHC). They are key physics objects for precision measurements and searches for new phenomena. This review provides an overview of the reconstruction and calibration of jets at the LHC during its first Run. ATLAS and CMS developed different approaches for the reconstruction of jets, but use similar methods for the energy calibration. ATLAS reconstructs jets utilizing input signals from their calorimeters and use charged particle tracks to refine their energy measurement and suppress the effects of multiple p-p interactions (pileup). CMS, instead, combines calorimeter and tracking information to build jets from particle flow objects. Jets are calibrated using Monte Carlo (MC) simulations and a residual in situ calibration derived from collision data is applied to correct for the differences in jet response between data and Monte Carlo. Large samples of dijet, Z+jets, and photon+jet events at the LHC allowed the calibration of jets with high precision, leading to very small systematic uncertainties. Both ATLAS and CMS achieved a jet energy calibration uncertainty of about 1% in the central detector region and for jets with transverse momentum pT>100 GeV. At low jet pT, the jet energy calibration uncertainty is less than 4%, with dominant contributions from pileup, differences in energy scale between quark and gluon jets, and jet flavor composition.

==> boostedsymbols.tex <==
%
% User-defined latex commands for SUBSTRUCTURE
%

\RequirePackage{xspace}

% Jet mass related
\newcommand{\mjet}      {\ensuremath{m^{\rm jet}}\xspace}
\newcommand{\mlead}     {\ensuremath{\mjet_{1}}\xspace}
\newcommand{\mleadavg}  {\ensuremath{\langle\mlead\rangle}\xspace}
\newcommand{\Mjet}      {\mjet}
\newcommand{\massjet}   {\mjet}
\newcommand{\masscorr}  {\ensuremath{m^{\rm corr}}}
\newcommand{\mThresh}   {\ensuremath{M_{\rm threshold}}\xspace}
\newcommand{\mjetAvg}   {\ensuremath{\langle\mjet\rangle}\xspace}
\newcommand{\masstrkjet}{\ensuremath{m^{\rm track \; jet}}\xspace}

\newcommand{\Wmass}     {\ensuremath{m_{\Wboson}}\xspace}
\newcommand{\WmassT}    {\ensuremath{m^{\Wboson}_{T}}\xspace}
\newcommand{\topmass}   {\ensuremath{m_{\rm top}}\xspace}
\newcommand{\massZprime}{\ensuremath{m_{\Zprime}}\xspace}

% Jet algorithm and grooming related
\newcommand{\akt}       {\antikt\xspace}
\newcommand{\Akt}       {\Antikt\xspace}
\newcommand{\AKT}       {\akt}
\newcommand{\AKTFat}    {\antikt, \ensuremath{R=1.0}\xspace}
\newcommand{\AKTPrune}  {\antikt, \ensuremath{R=1.0} (pruned)\xspace}
\newcommand{\AKTFilt}   {\antikt, \ensuremath{R=1.0} (filtered)\xspace}
\newcommand{\KTSix}     {\ensuremath{k_{t}}, \ensuremath{R=0.6}\xspace}
\newcommand{\kt}        {\ensuremath{k_{t}}\xspace}
\newcommand{\ca}        {Cambridge-Aachen\xspace}
\newcommand{\CamKt}     {\ensuremath{\mathrm{C/A}}\xspace}
\newcommand{\CASix}     {\CamKt, \ensuremath{R=0.6}\xspace}
\newcommand{\CAFat}     {\CamKt, \ensuremath{R=1.2}\xspace}
\newcommand{\CAPrune}   {\CamKt, \ensuremath{R=1.2} (pruned)\xspace}
\newcommand{\CAFilt}    {\CamKt, \ensuremath{R=1.2} (filtered)\xspace}
\newcommand{\SISCone}   {SISCone}
\newcommand{\SISConeSiz}{\SISCone, \ensuremath{R=0.6}\xspace}
\newcommand{\minKt}     {\ensuremath{\min\left(\pti^2, \ptj^2\right)}\xspace}
\newcommand{\minAKt}    {\ensuremath{\min\left(\pti^{-2}, \ptj^{-2}\right)}\xspace}
\newcommand{\minGen}    {\ensuremath{\min\left(\pti^{2p}, \ptj^{2p}\right)}\xspace}
\newcommand{\Rij}       {\ensuremath{R_{ij}}\xspace}
\newcommand{\DRij}      {\ensuremath{\Delta\Rij}\xspace}
\newcommand{\DRratio}   {\ensuremath{\frac{\DRij^2}{R^2}}\xspace}
\newcommand{\diB}       {\ensuremath{d_{iB}}\xspace}
\newcommand{\Rfilt}     {\ensuremath{R_{\rm filt}}\xspace}
\newcommand{\jone}      {\ensuremath{J_{1}}\xspace}
\newcommand{\jtwo}      {\ensuremath{J_{2}}\xspace}
\newcommand{\sjone}     {\ensuremath{j_{1}}\xspace}
\newcommand{\sjtwo}     {\ensuremath{j_{2}}\xspace}
\newcommand{\msubjone}  {\ensuremath{m^{\sjone}}\xspace}
\newcommand{\msubjtwo}  {\ensuremath{m^{\sjtwo}}\xspace}
\newcommand{\mjone}     {\ensuremath{m^{\jone}}\xspace}
\newcommand{\mjtwo}     {\ensuremath{m^{\jtwo}}\xspace}
\newcommand{\ptsubjone} {\ensuremath{p_{T}^{\sjone}}\xspace}
\newcommand{\ptsubjtwo} {\ensuremath{p_{T}^{\sjtwo}}\xspace}
\newcommand{\Rsubjets}  {\ensuremath{R_{\sjone,\sjtwo}}\xspace}
\newcommand{\DRsubjets} {\ensuremath{\Delta\Rsubjets}\xspace}
\newcommand{\pti}       {\ensuremath{p_{{\rm T}i}}\xspace}
\newcommand{\ptj}       {\ensuremath{p_{Tj}}\xspace}
\newcommand{\ycut}      {\ensuremath{y_{\rm cut}}\xspace}
\newcommand{\mcut}      {\ensuremath{m_{\rm cut}}\xspace}
\newcommand{\ymin}      {\ensuremath{y_{\min}}\xspace}
\newcommand{\fcut}      {\ensuremath{f_{\rm cut}}\xspace}
\newcommand{\Rsub}      {\ensuremath{R_{\rm sub}}\xspace}
\newcommand{\drsub}     {\ensuremath{\Rsub}\xspace}
\newcommand{\mufrac}    {\ensuremath{\mu_{\rm frac}}\xspace}
\newcommand{\rcut}      {\ensuremath{R_{\rm cut}}\xspace}
\newcommand{\zcut}      {\ensuremath{z_{\rm cut}}\xspace}
\renewcommand{\pt}      {\ensuremath{p_{\rm T}}\xspace}
\renewcommand{\pttrue}  {\ensuremath{p_{\rm T}^{\rm true}}\xspace}
\newcommand{\largeR}    {large-\ensuremath{R}\xspace}
\newcommand{\LargeR}    {Large-\ensuremath{R}\xspace}
\newcommand{\NjetStd}   {\ensuremath{N_{\rm jet}^{R4}}\xspace}


% Insitu mass validation
\newcommand{\rtrkjet}       {\ensuremath{r_{\rm track \; jet}}\xspace}
\newcommand{\rtrkjetPt}     {\ensuremath{\rtrkjet^{p_T}}\xspace}
\newcommand{\rtrkjetM}      {\ensuremath{\rtrkjet^{M}}\xspace}
\newcommand{\rtrkjetPtData} {\ensuremath{\rtrkjet^{p_{T},{\rm data}}}\xspace}
\newcommand{\rtrkjetMData}  {\ensuremath{\rtrkjet^{M,{\rm data}}}\xspace}
\newcommand{\rtrkjetPtMC}   {\ensuremath{\rtrkjet^{p_{T},{\rm MC}}}\xspace}
\newcommand{\rtrkjetMMC}    {\ensuremath{\rtrkjet^{M,{\rm MC}}}\xspace}
\newcommand{\RtrkjetPt}     {\ensuremath{R_{r{\rm \; track \; jet}}^{p_T}}\xspace}
\newcommand{\RtrkjetM}      {\ensuremath{R_{r{\rm \; track \; jet}}^{M}}\xspace}

% Jet substructure related
\newcommand{\shapeV}    {\ensuremath{{\cal V}}\xspace}
\newcommand{\subjetpt}  {\ensuremath{p_{T}^{\rm subjet}}\xspace}
\newcommand{\yij}       {\ensuremath{y_{ij}}\xspace}
\newcommand{\dcut}      {\ensuremath{d_{\rm cut}}\xspace}
\newcommand{\dmin}      {\ensuremath{d_{\min}}\xspace}
\newcommand{\dij}       {\ensuremath{d_{ij}}\xspace}
\newcommand{\Dij}       {\ensuremath{\sqrt{\dij}}\xspace}
\newcommand{\DOneTwo}   {\ensuremath{\sqrt{d_{12}}}\xspace}
\newcommand{\DTwoThr}   {\ensuremath{\sqrt{d_{23}}}\xspace}
\newcommand{\yOneTwo}   {\ensuremath{y_{1}}\xspace}
\newcommand{\yTwoThr}   {\ensuremath{y_{2}}\xspace}
\newcommand{\yOneTwoDef}{\ensuremath{\yOneTwo=\DOneTwo/\mjet}\xspace}
\newcommand{\yTwoThrDef}{\ensuremath{\yTwoThr=\DTwoThr/\mjet}\xspace}
\newcommand{\xj}        {\ensuremath{x_{J}}\xspace}
\newcommand{\jetFunc}   {\ensuremath{J^{(eik),c} (\mjet,\pT,R)}\xspace}
\newcommand{\tauOne}    {\ensuremath{\tau_1}\xspace}
\newcommand{\tauTwo}    {\ensuremath{\tau_2}\xspace}
\newcommand{\tauThr}    {\ensuremath{\tau_3}\xspace}
\newcommand{\tauN}      {\ensuremath{\tau_N}\xspace}
\newcommand{\tauTwoOne} {\ensuremath{\tau_{21}}\xspace}
\newcommand{\tauThrTwo} {\ensuremath{\tau_{32}}\xspace}
\newcommand{\dip}       {\ensuremath{\mathcal{D}}\xspace}
\newcommand{\dipOneTwo} {\ensuremath{\dip_{12}}\xspace}
\newcommand{\dipTwoThr} {\ensuremath{\dip_{23}}\xspace}
\newcommand{\dipOneThr} {\ensuremath{\dip_{13}}\xspace}

% Samples
\newcommand{\Zprimett}  {\ensuremath{\Zprime\ra t\bar{t}}\xspace}
\newcommand{\Zqq}       {\ensuremath{Z\ra q\bar{q}}\xspace}
\newcommand{\Wqq}       {\ensuremath{W\ra q\bar{q}}\xspace}


% Random
\newcommand{\mpi}{multiple parton interactions\xspace} % David/Emily using multiple proton interactions.
                                                                                                                 
